Investigation of the Thermal Structure in the Atmospheric Boundary Layer During Evening Transition and the Impact of Aerosols on Radiative Cooling

We have explored the evening transition using data from eighty days of observations across two fog seasons at the Kempegowda International Airport, Bengaluru (KIAB). Through field experiments and simulations integrating aerosol interaction in a radiation-conduction model, we elucidate the impact of aerosols on longwave cooling of the Atmospheric Boundary Layer (ABL). Field observations indicate that under calm and clear-sky conditions, the evening transition typically results in a distinct vertical thermal structure called the Lifted Temperature Minimum (LTM). We observe that the prevailing profile near the surface post-sunset is the LTM-profile. Additionally, the occurrence of LTM is observed to increase with decreases in downward and upward longwave flux, soil sensible heat flux, wind speed, and turbulent kinetic energy measured at two meters above ground level (AGL). In such scenarios, the intensity of LTM-profiles is primarily governed by aerosol-induced longwave heating rate (LHR) within the surface layer. Furthermore, the presence of clouds leads to increased downward flux, causing the disappearance of LTM, whereas shallow fog can enhance LTM intensity, as observed in both field observations and simulations. Usually, prevailing radiation models underestimate aerosol-induced longwave heating rate (LHR) by an order, compared to actual field observations. We attribute this difference to aerosol-induced radiation divergence. We show that impact of aerosol-induced LHR extends hundreds of meters into the inversion layer, affecting temperature profiles and potentially influencing processes such as fog formation. As the fog layer develops, LHR strengthens at its upper boundary, however, we highlight the difficulty in detecting this cooling using remote instruments such as microwave radiometer.

==> header.tex <==
% Add any additional LaTeX packages and macros here
\usepackage{siunitx}

%---

\iflatexml
% Add any LateXML specific commands here

%---

\else
% The commands below will only change the exported PDF. Edit or remove as needed

\renewcommand{\sfdefault}{ptm}
\renewcommand{\familydefault}{\sfdefault}


\paperfield{Field of the paper}
\abbrevs{ABC, a black cat; DEF, doesn't ever fret; GHI, goes home immediately.}
\corraddress{Author One PhD, Department, Institution, City, State or Province, Postal Code, Country}
\corremail{correspondingauthor@email.com}
\presentadd{Department, Institution, City, State or Province, Postal Code, Country}
\fundinginfo{Funder One, Funder One Department, Grant/Award Number: 123456, 123457 and 123458; Funder Two, Funder Two Department, Grant/Award Number: 123459}
\fi

%---
